Modular Deep Reinforcement Learning for Continuous Motion Planning with Temporal Logic

This paper investigates the motion planning of autonomous dynamical systems modeled by Markov decision processes (MDP) with unknown transition probabilities over continuous state and action spaces. Linear temporal logic (LTL) is used to specify high-level tasks over infinite horizon, which can be converted into a limit deterministic generalized B\"uchi automaton (LDGBA) with several accepting sets. The novelty is to design an embedded product MDP (EP-MDP) between the LDGBA and the MDP by incorporating a synchronous tracking-frontier function to record unvisited accepting sets of the automaton, and to facilitate the satisfaction of the accepting conditions. The proposed LDGBA-based reward shaping and discounting schemes for the model-free reinforcement learning (RL) only depend on the EP-MDP states and can overcome the issues of sparse rewards. Rigorous analysis shows that any RL method that optimizes the expected discounted return is guaranteed to find an optimal policy whose traces maximize the satisfaction probability. A modular deep deterministic policy gradient (DDPG) is then developed to generate such policies over continuous state and action spaces. The performance of our framework is evaluated via an array of OpenAI gym environments.

==> modular_neural_network.tex <==
\usetikzlibrary{3d,decorations.text,shapes.arrows,positioning,fit,backgrounds}
\tikzset{pics/fake box/.style args={% #1=color, #2=x dimension, #3=y dimension, #4=z dimension
#1 with dimensions #2 and #3 and #4}{
code={
\draw[gray,ultra thin,fill=#1]  (0,0,0) coordinate(-front-bottom-left) to
++ (0,#3,0) coordinate(-front-top-right) --++
(#2,0,0) coordinate(-front-top-right) --++ (0,-#3,0) 
coordinate(-front-bottom-right) -- cycle;
\draw[gray,ultra thin,fill=#1] (0,#3,0)  --++ 
 (0,0,#4) coordinate(-back-top-left) --++ (#2,0,0) 
 coordinate(-back-top-right) --++ (0,0,-#4)  -- cycle;
\draw[gray,ultra thin,fill=#1!80!black] (#2,0,0) --++ (0,0,#4) coordinate(-back-bottom-right)
--++ (0,#3,0) --++ (0,0,-#4) -- cycle;
\path[gray,decorate,decoration={text effects along path,text={CONV}}] (#2/2,{2+(#3-2)/2},0) -- (#2/2,0,0);
}
}}
% from https://tex.stackexchange.com/a/52856/121799
\tikzset{circle dotted/.style={dash pattern=on .05mm off 2mm,
                                         line cap=round}}
                                     
    
    \begin{figure}[!t]\centering
	{{
	    \scalebox{1.2}{
        \begin{tikzpicture}[x={(1,0)},y={(0,1)},z={({cos(60)},{sin(60)})},
        font=\sffamily\small,scale=2]
        %
        % comment these out if you want to see where the axes point to
        % \draw[-latex] (0,0,0) -- (3,0,0) node[below]{$x$};
        % \draw[-latex] (0,0,0) -- (0,3,0) node[left]{$y$};
        % \draw[-latex] (0,0,0) -- (0,0,3) node[below]{$z$};
        % a plane
        %
        \node[draw,single arrow, orange,fill=orange!30] at (9.6,0.5,0) {$q_0\rightarrow q_1$};
        \node[draw,single arrow, orange,fill=orange!30] at (10.9,0.5,0) {$q_1\rightarrow q_2$};
        \node[draw,single arrow, orange,fill=orange!30] at (12.2,0.5,0) {$q_2\rightarrow q_3$};
        
        \node[circle,draw,blue,fill=blue!30] (A1) at (9,1,0) {~~~};
        \node[circle,draw,red,fill=red!30,below=4pt of A1] (A2) {~~~};
        \node[circle,draw,green,fill=green!30,below=18pt of A2] (A3) {~~~};
        \draw[circle dotted, line width=2pt,shorten <=3pt] (A2) -- (A3);
        
        \node[circle,draw,blue,fill=blue!30] (B1) at (10.3,1,0) {~~~};
        \node[circle,draw,red,fill=red!30,below=4pt of B1] (B2) {~~~};
        \node[circle,draw,green,fill=green!30,below=18pt of B2] (B3) {~~~};
        \draw[circle dotted, line width=2pt,shorten <=3pt] (B2) -- (B3);
        
        \node[circle,draw,blue,fill=blue!30] (C1) at (11.6,1,0) {~~~};
        \node[circle,draw,red,fill=red!30,below=4pt of C1] (C2) {~~~};
        \node[circle,draw,green,fill=green!30,below=18pt of C2] (C3) {~~~};
        \draw[circle dotted, line width=2pt,shorten <=3pt] (C2) -- (C3);
        
        \node[circle,draw,blue,fill=blue!30] (D1) at (12.9,1,0) {~~~};
        \node[circle,draw,red,fill=red!30,below=4pt of D1] (D2) {~~~};
        \node[circle,draw,green,fill=green!30,below=18pt of D2] (D3) {~~~};
        \draw[circle dotted, line width=2pt,shorten <=3pt] (D2) -- (D3);
        
        \begin{scope}[on background layer]
        \node[yellow,thick,rounded corners,fill=yellow!30,fit=(A1) (A3),label=above:$\textcolor{blue}{0}$,label=below:$\textcolor{black}{q_0}$]{};
        \node[orange,thick,rounded corners,fill=orange!30,fit=(B1) (B3),label=above:$\textcolor{blue}{\Phi_1}$, label=below:$\textcolor{black}{q_1}$]{};
        \node[orange,thick,rounded corners,fill=orange!30,fit=(C1) (C3),label=above:$\textcolor{blue}{\Phi_2}$,label=below:$\textcolor{black}{q_2}$]{};
        \node[red,thick,rounded corners,fill=red!50,fit=(D1) (D3),label=above:$\textcolor{blue}{1-r_F}$,label=below:$\textcolor{black}{q_3}$]{};
        \end{scope}
        
        \end{tikzpicture}

			}
			}}
		\caption{\label{fig:modular_DDPG} Demonstration of modular DDPG for LDGBA $\mathcal{A}_{\varphi_{P}}$} in shown Fig. \ref{fig:reward_shaping} 
	\end{figure}

